A Machine Learning Approach for Simultaneous Demapping of QAM and APSK Constellations

As telecommunication systems evolve to meet increasing demands, integrating deep neural networks (DNNs) has shown promise in enhancing performance. However, the trade-off between accuracy and flexibility remains challenging when replacing traditional receivers with DNNs. This paper introduces a novel probabilistic framework that allows a single DNN demapper to demap multiple QAM and APSK constellations simultaneously. We also demonstrate that our framework allows exploiting hierarchical relationships in families of constellations. The consequence is that we need fewer neural network outputs to encode the same function without an increase in Bit Error Rate (BER). Our simulation results confirm that our approach approaches the optimal demodulation error bound under an Additive White Gaussian Noise (AWGN) channel for multiple constellations. Thereby, we address multiple important issues in making DNNs flexible enough for practical use as receivers.

==> ExperimentalSetup/experimental_setup.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Experimental Setup/Kopie van literature-symbol-demapping.drawio.pdf}
    \caption{The system model used to evaluate our approach. For symbol demapping, we use a hard-decision demapper as a baseline and compare it to our DNN.}
    \label{fig:awgn-channel}
\end{figure}

\begin{table}[t]
\centering
\caption{Hyperparameters used for the simulations.}
\label{tab:hyperparameters}
\begin{tabular}{ll}
\toprule
\textbf{Name} & \textbf{Value} \\
\midrule
\# of Sequences &  $10000$ \\
Frame length & $2048$ \\
Noise Range (dB) & $-5 - 30$\\
Filter Rolloff & $0.25$\\
Filter Span & $10$\\
Optimiser & AdamW\cite{KingBa15, loshchilov2017decoupled} \\
Learning Rate & $0.003$ \\
Batch Size & $64\times $ \#Datasets \\
Number of Runs & $3$\\
Max Epochs & $100$ \\
\bottomrule
\end{tabular}
\end{table}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{Experimental Setup/u-net-architecture.png}
%    \caption{\arwin{PLACEHOLDER NEED TO REPLACE WITH OWN IMAGE} The U-Net architecture we use for our Deep Demapper. }
%    \label{fig:architecture}
%\end{figure}


To evaluate the performance of our method, we have opted to simulate data over a simple AWGN channel to better understand how our method behaves under various combinations of constellations. As an AWGN channel permits a simple optimal demodulation, we compare our method with it. The simulation pipeline is depicted in Fig. \ref{fig:awgn-channel}.

To perform our experiments, we use a simple DNN receiver. It consists of two hidden layers of size $256$ with a ReLU activation function and batch normalization. It has a linear output layer that generates the representation, after which we apply our method to generate the bit LLRs. We denote the settings used to run our experiments in Table \ref{tab:hyperparameters}. Out of the $10,000$ sequences per constellation, we use $1,000$ for testing, $1,000$ for validation, and $8,000$ for training.

For the AWGN channel, we sample uniform randomly from the range mentioned. We generate our APSK constellation based on the DVB-S2x specification \cite{morello2003}. These constellations are determined by the configuration and code rate. For example, the constellation $64$-APSK-7/9 is the APSK constellation associated with the code rate of 7/9 under this specification.


==> RelatedWorks/related_works.tex <==
As these distortions can be challenging to correct, multiple lines of work have been investigating the potential benefits of DNNs. The first line \cite{oshea2017ae, dorner2018ijstsp, xie2021huiqiang} uses an \emph{Auto Encoder} (AE) to model the entire transmitter-receiver pipeline. Through this end-to-end pipeline, all components can jointly learn to minimize the eventual error rate. However, this approach requires the sender and receiver to share a model and its parameters. While this may be practical in the future, the need for backwards compatibility could obstruct the adoption rate.

Second, \emph{deep channel estimation} (DCE) \cite{soltani2019icl, balevi2020, wang2021yazheng} replaces only the channel estimation and equalization components with deep neural networks. The advantage of this approach is that it allows leveraging the power of DNNs without sacrificing the modularity and partial interpretability of the communications system. In particular, the focus in this line of research also lies in minimizing the number of parameters and required computational resources.

However, DNNs are generally most accurate when modelling as many components in an end-to-end manner. That is a third line that \cite{honkala2021itwc, zhao2021zhongyuan, korpi2021} extends the neural network such that it also performs symbol demapping/demodulation. These works posit that doing so results in better performance through not relying on possibly unrealistic assumptions and instead learning the correct ones end-to-end.
